Robust Geometric Metric Learning

This paper proposes new algorithms for the metric learning problem. We start by noticing that several classical metric learning formulations from the literature can be viewed as modified covariance matrix estimation problems. Leveraging this point of view, a general approach, called Robust Geometric Metric Learning (RGML), is then studied. This method aims at simultaneously estimating the covariance matrix of each class while shrinking them towards their (unknown) barycenter. We focus on two specific costs functions: one associated with the Gaussian likelihood (RGML Gaussian), and one with Tyler's M -estimator (RGML Tyler). In both, the barycenter is defined with the Riemannian distance, which enjoys nice properties of geodesic convexity and affine invariance. The optimization is performed using the Riemannian geometry of symmetric positive definite matrices and its submanifold of unit determinant. Finally, the performance of RGML is asserted on real datasets. Strong performance is exhibited while being robust to mislabeled data.

==> contents/5_annexe.tex <==
\begin{itemize}
    \item principle of metric learning: \cite{Weinberger09} (LMNN) with the first paper \cite{Xing03distancemetric} (MMC) based on a Mahalanobis distance.
    \item Information-Theoretic Metric Learning (ITML) use a log det distance \cite{Davis07,Meyer11}
    \item a geometric interpretation is proprosed in \cite{Zadeh16}
    \item we propose to robustify its cost function by keeping the $g$-convexity property \cite{wiesel2012geodesic} and using some robust functions \cite{ollila2012complex}
    \item we also use a regularization term, ...
    \item test on real dataset like breizhcrops \cite{RPZLK20}
\end{itemize}

Let us consider weak-supervision, which is provided through the sets of pairs:
\begin{equation}
    \begin{array}{ll}
      \mathcal{S}:=   & \{(\mathbf{x}_i,\mathbf{x}_j)|\mathbf{x}_i \text{~and~} \mathbf{x}_j \text{~are in the same class} \}  \\
         \mathcal{D}:=   & \{(\mathbf{x}_i,\mathbf{x}_j)|\mathbf{x}_i \text{~and~} \mathbf{x}_j \text{~are in different classes} \} 
    \end{array}
\end{equation}
Denote $\mathbf{S}\in \mathbb{R}^{p \times n_s}$ and $\mathbf{D}\mathbb{R}^{p \times n_d}$,the matrices of sub sampled paired differences defined by
\begin{align}
    [\mathbf{S}]_{:,k} &= \mathbf{s}_k = \mathbf{x}_i - \mathbf{x}_j ,(\mathbf{x}_i,\mathbf{x}_j)\in \mathcal{S}\\
    [\mathbf{D}] _{:,k} &= \mathbf{d}_k = \mathbf{x}_i - \mathbf{x}_j ,(\mathbf{x}_i,\mathbf{x}_j)\in \mathcal{D}
\end{align}
In \cite{Zadeh16}, the formulation problem is:
\begin{equation}
\begin{array}{ll}
\underset{\boldsymbol{\Sigma}\in\mathcal{S}_{p}^{+}}{\rm minimize}
    & \sum_{i=1}^{n_s} \tr(\boldsymbol{\Sigma}\mathbf{s}_i\mathbf{s}_i^T)  + \sum_{i=1}^{n_d}  \tr(\boldsymbol{\Sigma}^{-1}\mathbf{d}_i\mathbf{d}_i^T)
\end{array}
    \label{eq:form_classic}
\end{equation}
Like in many papers on metric learning, they add a regularization term to shrink the solution towards a matrix $\boldsymbol{\Sigma}_0$ through the following distance:
\begin{equation}
    d(\boldsymbol{\Sigma},\boldsymbol{\Sigma}_0) = \text{tr}(\boldsymbol{\Sigma}\boldsymbol{\Sigma}_0^{-1})+\text{tr}(\boldsymbol{\Sigma}^{-1}\boldsymbol{\Sigma}_0)-2p
    \label{eq:distregul}
\end{equation}

We propose to robustify the cost function:
\begin{equation}
    \begin{array}{ll}
    \underset{\boldsymbol{\Sigma}\in\mathcal{S}_{p}^{+}}{\rm minimize} & \sum_{i=1}^{n_s} \rho(\mathbf{s}_i^T\boldsymbol{\Sigma}\mathbf{s}_i) 
      + \sum_{i=1}^{n_d} \rho(\mathbf{d}_i^T\boldsymbol{\Sigma}^{-1}\mathbf{d}_i)
    \end{array}
\label{eq:robustmetriclearning}
\end{equation}
Several functions for $\rho$ are possible:
\begin{itemize}
    \item $\rho(x)=x$ which is the classical case of \cite{Zadeh16} already given in \eqref{eq:form_classic},
    \item $\rho(x)=\log(1+x)$,
    \item $\rho(x)=\left\{ \begin{array}{ll}
         x  & x\leq c^2 \\
         c^2\log(x)+c^2(1-\log(c^2)) & x > c^2 
    \end{array}\right.$, which the Huber function
\end{itemize}
We notice that the $g$-convexity of \eqref{eq:robustmetriclearning} is kept if $\rho$ has following properties: ????. This is true for the previous functions of $\rho$ studied in the paper. Maybe we have to introduce the weighting of $\mathbb{S}$ and $\mathbf{D}$. 

\section{Solution and algorithm}

We first give in the following proposition the euclidean gradient.
\begin{Proposition}
The euclidean gradient of the cost function \eqref{eq:robustmetriclearning} (denoted here $f$) w.r.t. of $\boldsymbol{\Sigma}$ is:
\begin{equation}
\begin{array}{ll}
     \grad f (\Sigma) = & \sum_{i=1}^{n_s} \rho^{\prime}(\mathbf{s}_i^T\boldsymbol{\Sigma}\mathbf{s}_i)\mathbf{s}_i\mathbf{s}_i^T \\
     & - \boldsymbol{\Sigma}^{-1} \left(\sum_{i=1}^{n_d} \rho^{\prime}(\mathbf{d}_i^T\boldsymbol{\Sigma}^{-1}\mathbf{d}_i)\mathbf{d}_i\mathbf{d}_i^T \right) \boldsymbol{\Sigma}^{-1}
\end{array}
\label{eq:gradeuclidean}
\end{equation}
\end{Proposition}
From this derivation, we are able to provide the equation that the solution must respect:
\begin{equation}
    \begin{array}{ll}
     \boldsymbol{\Sigma} = & \left( \sum_{i=1}^{n_s} \rho^{\prime}(\mathbf{s}_i^T\boldsymbol{\Sigma}\mathbf{s}_i)\mathbf{s}_i\mathbf{s}_i^T\right)^{-1}  \boldsymbol{\Sigma}^{-1} \\
         & \left(\sum_{i=1}^{n_d} \rho^{\prime}(\mathbf{d}_i^T\boldsymbol{\Sigma}^{-1}\mathbf{d}_i)\mathbf{d}_i\mathbf{d}_i^T \right) 
    \end{array}
\end{equation}
From this equation, we conclude that a closed form is impossible to find for a general function $\rho$. A fixed point could be considered but without any proof on the convergence.

Therefore, we prefer to use a Riemaniann gradient descent algorithm to estimate the correct solution. Since the cost function is $g$-convex, we have the convergence proof that this algorithm ensures to find the optimal solution. To increase the speed of convergence that leans on the fisher information metric, the natural gradient is used \cite{AMS08}. 

To perform this algorithm, some geometric tools of the SPD manifold are needed. The tanget space $T_{\boldsymbol{\Sigma}}\mathcal{S}_p^{+}$ is identified to $\mathcal{S}_p$. A metric has to be chosen and it is well known that the most interesting is the Fisher information metric \cite{Smith05}:
\begin{equation}
    \langle \xi,\eta \rangle_{\boldsymbol{\Sigma}} = \frac{1}{p}\tr(\boldsymbol{\Sigma}^{-1}\xi\boldsymbol{\Sigma}^{-1}\eta)
    \label{eq:fim}
\end{equation}
To come back in the manifold, a retraction operator is used and for the SPD manifold, we resort to the exponential mapping operator:
\begin{equation}
    \exp_{\boldsymbol{\Sigma}}^{\mathcal{S}_p^{+}} (\xi) = \boldsymbol{\Sigma} \text{expm}(\boldsymbol{\Sigma}^{-1}\xi)
    \label{eq:expm}
\end{equation}
Finally we have to compute the Riemannian's gradient from the euclidean gradient and the metric \eqref{eq:fim} thanks to the following relation:
\begin{equation}
    \begin{array}{lll}
      <\grad_{\mathcal{S}_p^{+}} f,\xi>_{\boldsymbol{\Sigma}}   & = & <\grad f,\xi> 
    \end{array},
    \label{eq:defgradientR}
\end{equation}
where $<.,.>$ is the euclidean gradient. By identification and by using \eqref{eq:fim} and \eqref{eq:gradeuclidean}, we obtain for the Riemaniann gradient:
\begin{equation}
\begin{array}{ll}
     \grad_{\mathcal{S}_p^{+}} f (\Sigma) = & \boldsymbol{\Sigma}\left(\sum_{i=1}^{n_s} \rho^{\prime}(\mathbf{s}_i^T\boldsymbol{\Sigma}\mathbf{s}_i)\mathbf{s}_i\mathbf{s}_i^T\right)\boldsymbol{\Sigma} \\
     & - \sum_{i=1}^{n_d} \rho^{\prime}(\mathbf{d}_i^T\boldsymbol{\Sigma}^{-1}\mathbf{d}_i)\mathbf{d}_i\mathbf{d}_i^T 
\end{array}
\label{eq:gradriemann}
\end{equation}

Now, we are able to perform a Riemaniann gradient to obtain the solution of \eqref{eq:robustmetriclearning} and the algorithm is given in box \eqref{algo:RG}.

\begin{algorithm}
\KwIn{$\{(\mathbf{x}_i,\mathbf{x}_j)\}_{i,j} \in \mathcal{S},\mathcal{D}$, initialization $\boldsymbol{\Sigma}^{(0)}\in\mathcal{S}_{p}^{+}$, initial stepsize $\alpha_0>0$}
\KwOut{$\boldsymbol{\Sigma}$ in $\mathcal{S}_{p}^{+}$}
\For{$t=0$ \textbf{to convergence}}{
	$\boldsymbol{\Sigma}^{(t+1)} = \exp^{\mathcal{S}_{p}^{+}}_{\boldsymbol{\Sigma}^{(t)}}\left(\alpha_0^{t+1}\grad_{\mathcal{S}_{p}^{+}}f(\boldsymbol{\Sigma}^{(t)})\right)$
}
\caption{Gradient algorithm to metric learning of parameters of \eqref{eq:robustmetriclearning} in $\mathcal{S}_{p}^{+}$}
\label{algo:RG}
\end{algorithm}

If we add the regularization term in the cost function, the algorithm remains the same with an adding term in the Riemaniann gradient.

MDM ? Avec optim à faire avec la distance ? ou blanchiment ?
